Generalized Group Profiling for Content Customization

There is an ongoing debate on personalization, adapting results to the unique user exploiting a user's personal history, versus customization, adapting results to a group profile sharing one or more characteristics with the user at hand. Personal profiles are often sparse, due to cold start problems and the fact that users typically search for new items or information, necessitating to back-off to customization, but group profiles often suffer from accidental features brought in by the unique individual contributing to the group. In this paper we propose a generalized group profiling approach that teases apart the exact contribution of the individual user level and the "abstract" group level by extracting a latent model that captures all, and only, the essential features of the whole group. Our main findings are the followings. First, we propose an efficient way of group profiling which implicitly eliminates the general and specific features from users' models in a group and takes out the abstract model representing the whole group. Second, we employ the resulting models in the task of contextual suggestion. We analyse different grouping criteria and we find that group-based suggestions improve the customization. Third, we see that the granularity of groups affects the quality of group profiling. We observe that grouping approach should compromise between the level of customization and groups' size.

==> Figures_and_Charts.tex <==
\begin{figure}[!t]
\centering
\begin{tikzpicture}
\begin{axis}[
    width= 8.6cm, %\textwidth,
    height=7cm, %5cm,
    xmin=0,xmax=200,
%    ymin=0,ymax=1,
    grid = both,
    ylabel={MAP},
    xlabel={Group Size},
    scatter/classes={
	a={mark=square*,b},%
	b={mark=triangle*,r},%
	c={mark=o,draw=g},
	d={mark=pentagon*,draw=o}
	},
	]

	% \addplot[] is better than \addplot+[] here:
	% it avoids scalings of the cycle list
	\addplot[scatter,only marks,
		scatter src=explicit symbolic]
		coordinates {
			(9,0.2012)  [a]
			(44,0.2914) [a]
			(43,0.4181) [a]
			(45,0.2545)  [a]
			(15,0.2886)  [a]
			(14,0.2245)  [a]
			(8,0.1811)   [a]
			(23,0.3214) [a]
			(9,0.2012) [b]
			(87,0.2739) [b]
			(60,0.3855) [b]
			(22,0.3008) [b]
			(23,0.3214) [b]
			(96,0.2501) [c]
			(82,0.3300) [c]
			(23,0.3214) [c]
			(156,0.2418) [d]
			(46, 0.3633) [d]
		};
		\addplot[b,sharp plot,update limits=false] coordinates {(0,0.3003) (200,0.3003)} node[above] at (axis cs:165,0.3003) {\tiny{\textbf{0.3003}}}; 
		\addplot[r,sharp plot,update limits=false] coordinates {(0,0.3123) (200,0.3123)}node[above] at (axis cs:185,0.3123) {\tiny{\textbf{0.3123}}}; 
	    \addplot[g,sharp plot,update limits=false] coordinates {(0,0.2908) (200,0.2908)}node[above] at (axis cs:145,0.2908) {\tiny{\textbf{0.2908}}};  
		\addplot[o,sharp plot,update limits=false] coordinates {(0,0.2708) (200,0.2708)}node[above] at (axis cs:125,0.2708) {\tiny{\textbf{0.2708}}}; 
	
%	node[above] at (axis cs:0,0.26) {Houses};
		\legend{5-years,10-years,20-years,40-years}
\end{axis}
\end{tikzpicture}
\vspace{-12pt}
\caption{
Effect of groups granularity on the performance group profiling
 \label{fig:Chart2}}
 \vspace{-5pt}
 \end{figure}
 
     \definecolor{b}{HTML}{4981CE}
    \definecolor{g}{HTML}{859C27}
    \definecolor{r}{HTML}{B22222}
    \definecolor{o}{HTML}{FF6600}

\begin{figure}[!t]
\centering
\pgfplotsset{
    % #1: index in the group(0,1,2,...)
    % #2: number of plots of that group
    bar group size/.style 2 args={
        /pgf/bar shift={%
                % total width = n*w + (n-1)*skip
                % -> subtract half for centering
                -0.5*(#2*\pgfplotbarwidth + (#2-1)*\pgfkeysvalueof{/pgfplots/bar group skip})  + 
                % the '0.5*w' is for centering
                (.5+#1)*\pgfplotbarwidth + #1*\pgfkeysvalueof{/pgfplots/bar group skip}},%
    },
    bar group skip/.initial=2pt,
    plot 0/.style={fill=b, draw=b, pattern color = b, pattern = north east lines},%
    plot 1/.style={fill=g, draw=g, pattern color = g, pattern = north west lines},%
    plot 2/.style={fill=r, draw=r, pattern color = r, pattern = dots},%
}
\begin{tikzpicture}
    \begin{axis}[
       width= 8.6cm, %\textwidth,
        height=7cm, %5cm,
        ybar,%=0pt,
        bar width= 7pt,
        enlarge y limits=0.2,
        %grid = both,
        %x tick label style={/pgf/number format/1000 sep=},
        x tick label style={rotate=45,anchor=east},
    xtick=data,
    %legend style={at={(0.9,0.95),font=\fontsize{5}{6}},
    anchor=north,
    ylabel={MAP},
  legend style={at={(0.965,-0.28)}
  %legend style={at={(0.965,0.95),font=\fontsize{5}{6}}
  ,legend columns=-1},
    nodes near coords,
    every node near coord/.append style={font=\tiny, rotate=90, anchor=west},
    %nodes near coords align={vertical},
%    tick label style={font=\tiny}
            xtick={1,2,3,4,5,6,7},
            xticklabels={
            age,
            gender,
            group,
            t-type,
            t-duration,
            season,
            preferences
        },
        ]
                
\addplot[plot 0,bar group size={0}{2}]
        coordinates 
        {
(1,0.3123)
(2,0.2417)
(3,0.2989)
(4,0.2122)
(5,0.3971)
(6,0.2879)
};
        \addplot[plot 1,bar group size={1}{2}]
        coordinates {
(1,0.6713)
(2,0.5187)
(3,0.5811)
(4,0.5066)
(5,0.5799)
(6,0.5562)
};

        \addplot[plot 2,bar group size={0}{1}]
        coordinates {
(7,0.5136)
};


\legend{Group, Group+Preferences, Preferences}

\end{axis}
\end{tikzpicture}
\vspace{-4pt}
\caption{
Performance of employing user preferences\:-\:based and group-\:based customization on contextual suggestion task. Improvements of combining group-\:based and preferences\:-\:based approach over the preferences\:-\:based approach and corresponding group-\:based approaches are statistically significant based on one-tailed t-test, with p-value $<$ 0.05. \label{fig:Chart1}}
 \vspace{-5pt}
 \end{figure}



\newcommand*\rot{\rotatebox{90}}

\begin{table*}[!t]
\caption{\strut\label{tbl:stat} Statistics of users groups resulted by grouping based on different critera\strut}
\vspace{-10pt}
\small
\begin{tabularx}{\linewidth}{X|c@{~~}c@{~~}c@{~~}c@{~~}c|c@{~~}c|c@{~~}c@{~~}c@{~~}c|c@{~~}c@{~~}c|c@{~~}c@{~~}c@{~~}c|c@{~~}c@{~~}c@{~~}c}
\toprule
%\multirow{2}{*}{\textbf{Annotation labels} & \multicolumn{3}{c}{\textbf{Structural Aspects}}
\bf Grouping Criterion 
& \multicolumn{5}{c|}{\textbf{Age}} 
& \multicolumn{2}{c|}{\textbf{Gender}} 
& \multicolumn{4}{c|}{\textbf{Group Type}} 
& \multicolumn{3}{c|}{\textbf{Trip Type}} 
& \multicolumn{4}{c|}{\textbf{Trip Duration}} 
& \multicolumn{4}{c}{\textbf{Season}}
\\
\midrule
Groups &
\rot{$<20$} & \rot{$20-30$} & \rot{$30-40$} & \rot{$40-50$} & \rot{$>50$} & \rot{male} & \rot{female} & \rot{alone} & \rot{family} & \rot{friends} & \rot{other} & \rot{holiday} & \rot{business} & \rot{other} & \rot{night out} & \rot{day trip} & \rot{weekend} & \rot{longer} & \rot{spring} & \rot{summer} & \rot{autumn} & \rot{winter}
\\
\midrule
Group Size (\#users) &
 9 & 87 & 60 & 22 & 23 & 107 & 91 & 23 & 101 & 65 & 4 & 176 & 7 & 12 & 8 & 17 & 99 & 74 & 20 & 99 & 52 & 22
\\
\bottomrule
\end{tabularx}
\end{table*}


\begin{equation}
p(t|\theta_c) = \frac{c(t,C)}{\sum_{t' \in V} c(t',C)}
\end{equation}


\begin{equation}
P(t|\theta_s) = \sum_{u_i\in G} \bigg(P(t|\theta_{u_i}) \prod_{\substack{u_j\in G \\ j \neq i}} (1-P(t|\theta_{u_j}))\bigg) \cdot idf(t)
\label{eq:Spec}
\end{equation}

\begin{description}
\item[E-Step]
\begin{equation}
p(X_{u,t} = x) = \frac{\lambda_{u,x} p(t|\theta_x)}{\sum_{x' \in \{g,c,s\}}\lambda_{u,x'} p(t|\theta_x')}
\end{equation}
\item[M-Step]
\begin{equation}
p(t|\theta_g) = 
\frac{\sum_{u \in G}c(t,u) p(X_{u,t} = g)}{\sum_{t' \in V}\sum_{u \in G}c(t',u) p(X_{u,t'} = g)}
\end{equation}
\begin{equation}
\lambda_{u,x} = 
\frac{\sum_{t \in V}c(t,u) p(X_{u,t} = x)}{\sum_{x' \in \{g,c,s\}}\sum_{t \in V}c(t,u) p(X_{u,t} = x')}
\end{equation}
\end{description}
